Agnostic PAC Learning of k-juntas Using L2-Polynomial Regression

Many conventional learning algorithms rely on loss functions other than the natural 0-1 loss for computational efficiency and theoretical tractability. Among them are approaches based on absolute loss (L1 regression) and square loss (L2 regression). The first is proved to be an \textit{agnostic} PAC learner for various important concept classes such as \textit{juntas}, and \textit{half-spaces}. On the other hand, the second is preferable because of its computational efficiency, which is linear in the sample size. However, PAC learnability is still unknown as guarantees have been proved only under distributional restrictions. The question of whether L2 regression is an agnostic PAC learner for 0-1 loss has been open since 1993 and yet has to be answered. This paper resolves this problem for the junta class on the Boolean cube -- proving agnostic PAC learning of k-juntas using L2 polynomial regression. Moreover, we present a new PAC learning algorithm based on the Boolean Fourier expansion with lower computational complexity. Fourier-based algorithms, such as Linial et al. (1993), have been used under distributional restrictions, such as uniform distribution. We show that with an appropriate change, one can apply those algorithms in agnostic settings without any distributional assumption. We prove our results by connecting the PAC learning with 0-1 loss to the minimum mean square estimation (MMSE) problem. We derive an elegant upper bound on the 0-1 loss in terms of the MMSE error and show that the sign of the MMSE is a PAC learner for any concept class containing it.

==> FourierGeneralization.tex <==

\section{Generalized Fourier Algorithm }\label{subsec:orth}
\subsection{Fourier Orthogonalization} 
Next, we present the Gram-Schmidt process. First, we present this process for known but arbitrary distribution $D$. Then we discuss its empirical implementations for unknown $D$. %\addvb{The orthognolaziation process is described as in the following.}
  Let $\set{\sigma_1, \sigma_2, ..., \sigma_d}$ be a random permutation of $[d]$.  Fix the following ordering of subsets: 
\begin{align*}
&\emptyset, \{\sigma_1\}, \{\sigma_2\}, \{\sigma_1, \sigma_2\}, \{\sigma_3\}, \{\sigma_1, \sigma_3\}, \{\sigma_2, \sigma_3\}, \{\sigma_1, \sigma_2, \sigma_3\}, \cdots,\\\numberthis\label{eq:subset_ordering}
&\{\sigma_d\}, \{\sigma_1, \sigma_d\}, \{\sigma_2, \sigma_d\},  \cdots, \{\sigma_1, \sigma_2, ..., \sigma_d\}.
\end{align*}
Note that this ordering is increasing in the size of the subsets. At each step a new element $\{j_\ell\}$ is added together with all the subsets from the previous elements and  $j_\ell$. This process continues to complete all the elements of $[d]$. 

Next, we apply a Gram-Schmidt-type process on the monomials with the above ordering. Recall that the monomial corresponding to a subset $\mathcal{S}\subseteq[d]$ is denoted as $\chi_{\mathcal{S}}\equiv \prod_{j \in \mathcal{S}}x_j$.
 The first element in the orthogonalization is trivially given by $\ptset{\emptyset}\equiv 1$.  The $j$th basis function ($\ptSj$) corresponding to the $j$th subset ($\mathcal{S}_j$) in the above ordering is obtained from the following recursive operation:
%\vspace{-10pt}
\begin{align}\label{eq:GramSchmidt}
 \ptildSj \equiv \pSj- \sum_{\ell =1}^{j-1} \<\ptSl,\pSj\>_D ~ \ptSl, \qquad
  \ptSj \equiv \left\{ \begin{array}{ll}
 \frac{\ptildSj}{\norm{\ptildSj}_{2,D}} & \text{if}~ \norm{\ptildSj}_{2,D}>0,\\
  0 & \text{otherwise.}
 \end{array}  \right.
 \end{align}
% where $\norm{\ptildSj}_{2,D} = \sqrt{\<\ptildSj,\ptildSj\>_D}$.
As an example, consider the trivial permutation of $[d]$ with $\sigma_j=j$. Then, the second subset in \eqref{eq:subset_ordering} is $\mathcal{S}_2=\{1\}$. Hence, the second basis function is given by 
%\begin{equation*}
 $   \ptset{\mathcal{S}_2} \equiv \frac{x_{1}-\EE[X_{1}]}{\text{var}(X_1)},$
%\end{equation*}
where we used \eqref{eq:GramSchmidt}. 

 Note that the process in \eqref{eq:GramSchmidt} is for known $D$. Next, we adopt this process for agnostic setting where $D$ is unknown. For that, we apply the process in \eqref{eq:GramSchmidt} but with $D$ replaced by the $\Demp$, the empirical distribution corresponding to the training samples. In this case, the empirical orthogonalization running on the samples gives an estimate of the true orthogonalization with known $D$. This empirical process is implemented using a set of recursive formulas as described in Procedure \ref{proc:orthogonalization}.  %Once the orthogonal basis is obtained, the Fourier algorithm computes the empirical estimate of $\<Y,\pS\>_D$. %This is demonstrated as Algorithm \ref{alg:fourier}.
%  \red{\bf SPA: I would bring Algorithm 3 here.}
 
% \setcounter{algorithm}{0}
%\floatname{algorithm}{Procedure}
%\begin{algorithm}[h]
%
%\caption{ \textsc{FourierOrth}}
%\label{proc:orthogonalization}
%%\DontPrintSemicolon
%%\LinesNumbered
%\begin{algorithmic}
%\STATE {\bfseries Input:} {Samples $\{\bfx_\ell\}_{\ell=1}^n$,  depth parameter $k$, threshold $\varepsilon \in (0,1)$}
%
%%\SetKwFunction{ORTH}{FourierOrth}
%%\SetKwProg{Fn}{Procedure}{:}{} 
%%\SetKwProg{ORTH}{\textsc{Fourier-Orth}}{:}{}
%%\State Group the features into clusters of approximately $m$ features.
%%\State For each cluster perform the following procedure:  
%%Randomly partition the features into groups of size $m$. 
%%\Fn{\ORTH}{
%% Compute the empirical mean $\hat{\mu}_j$ and standard deviation $\hat{\sigma}_j$ of each feature. \;
%%\STATE \textsc{FourierOrth}:
%\STATE Generate all subsets $\mathcal{S}_j\subseteq [d]$ with size at most $k$ and with the standard ordering as in \eqref{eq:subset_ordering}.
%
%\STATE Compute the covariance matrix $\mathbf{\hat{B}}$ with elements: 
% $\hat{b}_{j,i}\gets \frac{1}{n}\sum_{\ell=1}^n  \chi_{\mathcal{S}_j}(\bfx_\ell)\chi_{\mathcal{S}_i}(\bfx_\ell).$
%%\pestsubset{\mathcal{S}_i}(\bfx_l)\pestsubset{\mathcal{S}_j}(\bfx_l)
%\STATE Set $\mathbf{\hat{A}}\gets \mathbf{\hat{B}}$.
%
%\FOR{row $j$ of $\mathbf{\hat{A}}$}
% \STATE Update the $j$th row: $\hat{\bfA}_{j,*}\gets \hat{\bfA}_{j,*}-\sum_{\ell<j} \hat{a}_{\ell,j} \hat{\bfA}_{\ell,*}$ 
%
% \STATE Compute $\nu_j \gets \hat{b}_{j,j}-\sum_{\ell<j} \hat{a}_{\ell,j}^2$\;
%
%\IF{$\nu_j\geq {\varepsilon}$}
%
%\STATE Normalize the $j$th row:  $
%\hat{\bfA}_{j,*}\gets \frac{\hat{\bfA}_{j,*}}{\sqrt{\nu_j}}$
%
%\STATE Set $\ptSj \equiv \frac{1}{\sqrt{\nu_j}}(\pSj- \sum_{\ell < j } \hat{a}_{\ell,j} ~ \psi_{\mathcal{S}_\ell})$
%
%\ELSE
%\STATE Set the $j$th row of $\hat{\bfA}$ zero: $\hat{\bfA}_{j,*}\gets \mathbf{0}$
%
%\STATE Set $\ptSj\equiv 0$
%\ENDIF
%   \ENDFOR
%
%
%
%
%%\State Each feature's measure equals: $\optfont{redundant}(j)\gets \optfont{norm}(\{j\})$ 
%%\State Rank the features based on $\optfont{measure}$. The features with $\optfont{measure}(i)\leq \epsilon^2$ declared as redundant. 
%
%\STATE all $\ptSj$'s.
%
%\end{algorithmic}
%\end{algorithm}

% \setcounter{algorithm}{0}
%\floatname{algorithm}{Procedure}
\begin{algorithm}[h]

\caption{ \textsc{FourierOrth}}
\label{proc:orthogonalization}
%\DontPrintSemicolon
%\LinesNumbered
\DontPrintSemicolon
\KwIn{Samples $\{\bfx_\ell\}_{\ell=1}^n$,  depth parameter $k$, threshold $\varepsilon \in (0,1)$.}
 \SetKwProg{Fn}{}{:}{} 
 \SetKwFunction{main}{LearningAlgorithm}
 \Fn{\main}{ 
Generate all subsets $\mathcal{S}_j\subseteq [d]$ with size at most $k$ and with the standard ordering as in \eqref{eq:subset_ordering}.\;
 Compute the covariance matrix $\mathbf{\hat{B}}$ with elements: 
 $\hat{b}_{j,i}\gets \frac{1}{n}\sum_{\ell=1}^n  \chi_{\mathcal{S}_j}(\bfx_\ell)\chi_{\mathcal{S}_i}(\bfx_\ell).$\;
%\pestsubset{\mathcal{S}_i}(\bfx_l)\pestsubset{\mathcal{S}_j}(\bfx_l)
 Set $\mathbf{\hat{A}}\gets \mathbf{\hat{B}}$.\;

\For{row $j$ of $\mathbf{\hat{A}}$}{
 Update the $j$th row: $\hat{\bfA}_{j,*}\gets \hat{\bfA}_{j,*}-\sum_{\ell<j} \hat{a}_{\ell,j} \hat{\bfA}_{\ell,*}$ \;

 Compute $\nu_j \gets \hat{b}_{j,j}-\sum_{\ell<j} \hat{a}_{\ell,j}^2$\;

\If{$\nu_j\geq {\varepsilon}$}{

Normalize the $j$th row:  $
\hat{\bfA}_{j,*}\gets \frac{\hat{\bfA}_{j,*}}{\sqrt{\nu_j}}$\;
 Set $\ptSj \equiv \frac{1}{\sqrt{\nu_j}}(\pSj- \sum_{\ell < j } \hat{a}_{\ell,j} ~ \psi_{\mathcal{S}_\ell})$\;
\Else{
 Set the $j$th row of $\hat{\bfA}$ zero: $\hat{\bfA}_{j,*}\gets \mathbf{0}$\;
 Set $\ptSj\equiv 0$\;
}
}
}
all $\ptSj$'s.
}
\end{algorithm}



==> Proofs/mean_est_effect.tex <==
\section{Proof of Lemma \ref{lem:Pi_Y est}}\label{proof:Pi_Y est}
%\section{The Effect of Estimating Features' Mean and Variance}\label{appx:mean_+variance_est}
%For any subset $\mathcal{S}\subseteq [d],$ let $\bfx^{\mathcal{S}}= \prod_{r\in \mathcal{S}}x_r$.
%Let $b_{j\ell} = \EE_D[\bfX^{\mathcal{S}_j}\bfX^{\mathcal{S}_{\ell}}]$ and  $\hat{b}_{j,\ell}= \frac{1}{n}\sum_{l=1}^n \bfx^{\mathcal{S}_j}\bfx^{\mathcal{S}_{\ell}}$ for all $j,\ell$ as in Procedure \ref{proc:orthogonalization}. Note that if $\hat{b}_{j,\ell}=b_{j,\ell}$ then $\ptS = \pestS$. Let $\Pibar$ denote the version of $\PiestJ$ under this assumption.    From Minkowsky's inequality, by adding and subtracting $\Pibar$ we have
%\begin{align}\label{eq:V+W}
%\norm{\PiJ-\PiestJ}_2 \leq \norm{\PiJ-\Pibar}_2+\norm{\Pibar-\PiestJ}_2.
%\end{align}
%Note that the first term above measures the error in estimating the Fourier coefficients; while the second term measures the error is creating the basis. 
%The first term is bounded as follows.
%
%%\begin{lem}\label{lem:fbarJbar-fJbar} 
%%Given any $\delta>0$, the inequality 
%%$\norm{\Piy-\Pibar}_2 \leq \sqrt{\frac{2 d^k c_k}{(k-1)!n }\log \frac{2d^k}{(k-1)!\delta}}$ holds with probability $(1-\delta)$.
%%\end{lem}
\input{Proofs/proof_lem_est_norm2.tex}
%Next, we bound the second term in \eqref{eq:V+W}. The argument follows from having $\hat{b}_{j,\ell}\approx b_{\ell,j}$ that itself follows again from McDiarmid's inequality. Since there are at most $O(d^k)$ such coefficients, we obtain a similar bound as in \eqref{eq:bound on V} for the second term. That said, combining all the bounds, we obtain the desired result
%\begin{align*}
%\norm{\PiJ-\PiestJ}_2 \leq O\bigg(\sqrt{\frac{ 2^k c_k}{n }\log \frac{d^k}{(k-1)!\delta}}\bigg),
%\end{align*}
%for any $k$-element subset $\mathcal{J}$. With that the proof is complete.
%
%\begin{customlem}{\ref{lem:imscore and 1norm}}[General Version]\label{lem:imscore and 1norm_adjusted}
% Given $\epsilon_0, \delta_0, \epsilon_1, \delta_1 \in (0,1)$, with probability at least $(1-\delta_1-\delta_0)$, the inequalities
% $$\Big|~ \imscore_1(\mathcal{J})- \norm{\fJ}_1~ \Big|\leq \epsilon_1+\lambda(\epsilon_0)$$ hold for all subsets $\mathcal{J}\subseteq [d]$ with size $k$, provided that  the number of training samples are atleast 
%$n_1(\epsilon_1, \delta_1)+m(\epsilon_0,\delta_0),$ where $n_1$ and $m$ are defined in Lemma \ref{lem:imscore and 1norm} and \ref{lem:mean_var_error}, respectively. 
%\end{customlem}
%
%\begin{customlem}{\ref{lem:fbarJbar-fJbar}}[General Version] \label{lem:fbarJbar-fJbar_adjusted}
%Given $\epsilon_0, \delta_0, \epsilon_1, \delta_1 \in (0,1)$, with probability at least $(1-\delta_2-\delta_0)$, the inequalities $$\norm{\fJ-\festJ}_2 \leq \epsilon_2+\lambda(\epsilon_0) $$ hold for all subsets $\mathcal{J}\subseteq [d]$ with size $k$, provided that the number of training samples are atleast {$n_2(\epsilon_2,\delta_2)+m(\epsilon_0,\delta_0)$}, where $n_2$ and $m$ are defined in Lemma \ref{lem:fbarJbar-fJbar} and \ref{lem:mean_var_error}, respectively. 
%\end{customlem}




==> Proofs/proof_cor_Fourier.tex <==
\section{Proof of Corollary \ref{cor:Fourier PAC}}
From the definition of $c_k$, we can write 
\begin{align*}
c_k&=\max_{\mathcal{S}: |\mathcal{S}|\leq k} \max_{\bfx \in \pmm^d} |\ps(\bfx)|^2\leq \max_{\mathcal{S}: |\mathcal{S}|\leq k} \prod_{j\in\mathcal{S}}\frac{(1+|\mu_j|)^2}{\sigma^2_j}\\
&= \max_{\mathcal{S}: |\mathcal{S}|\leq k} \prod_{j\in\mathcal{S}}\frac{1}{{1-|\mu_j|}},
\end{align*}
where the first inequality is from the definition of $\ps$. The laste quality holds as $\sigma_j^2=1-\mu_j^2$. Therefore, under the assumption that  $|\mu_j|\leq 1-\frac{1}{k}$, the following inequality holds
\begin{align*}
c_k \leq  \max_{\mathcal{S}: |\mathcal{S}|\leq k}  \prod_{j\in\mathcal{S}}{k}\leq k^{k}
\end{align*}
Hence, 
\begin{align*}
\frac{c_k}{(k-1)!}\leq \frac{k k^k}{k!}=2^{(k+1)\log_2 k -\log_2 k!}
\end{align*}
From Stirling approximation $\log_2 k! = k\log_2 k - k\log_2 e +O(\log_2 k)$. Hence, 
\begin{align*}
\frac{c_k}{(k-1)!}\leq 2^{k\log_2 e+ O(\log_2 k)}=e^k+O(k).
\end{align*}
Using the above inequality and Theorem \ref{thm:low degree concentrated} in the main text, we obtain the corollary. 
% that the generalization error of the algorithm is bounded from above by the following 
%\begin{align*}
%2\Pek+2\epsilon +O\Big(\sqrt{\frac{ d^k c_k}{(k-1)!n }\log\frac{4d^k}{(k-1)!\delta}}\Big)\leq 2\Pek+2\epsilon +O\Big(\sqrt{\frac{ d^k (e^k+O(k))}{n }\log\frac{4d^k}{(k-1)!\delta}}\Big),
%\end{align*}
%Also note that 
%\begin{align*}
%\log\frac{d^k}{(k-1)!}&= \log \frac{kd^k}{k!}=k\log_2d+\log_2k-k\log_2 k + k\log_2 e +O(\log_2 k)\\
%&=k\log_2\frac{ed}{k}  +O(\log_2 k)
%\end{align*}
%\begin{align*}
%O\Big(\sqrt{\frac{ k(ed)^k}{n }\Big(k\log_2\frac{ed}{k}  +O(\log_2 k)+\log \frac{4}{\delta}\Big)}\Big)=O\Big(\sqrt{\frac{ k(ed)^k}{n }\Big(k\log_2\frac{ed}{k}  +\log \frac{4k}{\delta}\Big)}\Big)
%\end{align*}


==> Proofs/proof_lem_est_norm2.tex <==
%\subsection{Proof of Lemma \ref{lem:fbarJbar-fJbar}} \label{proof:lem_fJbar}

%\begin{proof}
Recall that $\Pibar$ equals to $\Pibar(\bfx)= \sum_{\mathcal{S}\subseteq \mathcal{J}} \fbarS \pS(\bfx),$
where $ \fbarS$ are the estimated Fourier coefficients and are given as $\fbarS = \frac{1}{n}\sum_{i} Y(i) \pS(X(i)).$ In addition, by definition of the projection function $\PiJ$, we have that $\PiJ(\bfx)= \sum_{\mathcal{S}\subseteq \mathcal{J}} \fS~\pS(\bfx)$. Therefore, from Parseval's identity, the $2$-norm factors as 
\begin{align*}
\norm{\Piy-\Pibar}_2^2&=\sum_{\mathcal{S}\subseteq \mathcal{J}} |\fS-\fbarS|^2.
\end{align*}
In what follows, we show that $|\fS-\fbarS|\leq \epsilon$ for all subsets $\mathcal{S}\subseteq [d]$ with $|\mathcal{S}|\leq k$. For that, we use the standard arguments using McDiarmid's inequality. 

Note that $\fbarS$ is a function of the training random samples $(X(i), Y(i)), i=1,2,...,n$. Observe that $\EE[\fbarS]=\fS$ which implies that $\fbarS$ is an unbiased estimation of $\fS$. Since the samples are drawn \ac{iid},  we apply McDiarmid's inequality to bound the probability of the event  $|\fS-\fbarS|\geq \epsilon'$. 

For that, fix $i\in [d]$ and suppose $(\bfX(i), Y(i))$ in the training set is replaced with an \ac{IID} copy $(\tilde{\bfX}(i), \tilde{Y}(i))$. With this replacement $\fbarS$ is changed to another random variable denoted by $\tilde{f}_{ S} $. Then 
\begin{align*}
 |\fbarS-\tilde{f}_{ S} |&= \frac{1}{n} |Y(i)\pS({\bfX}(i))-\tilde{Y}(i)\pS(\tilde{\bfX}(i))|\\
 &\leq \frac{1}{n} |Y(i)\pS({\bfX}(i))|+|\tilde{Y}(i)\pS(\tilde{\bfX}(i))|\\
  &\leq \frac{1}{n} |\pS({\bfX}(i))|+|\pS(\tilde{\bfX}(i))|\\
 &\leq \frac{2}{n} \abs{\prod_{j\in \mathcal{S}}X_j(i)}=\frac{2}{n},
 \end{align*} 
Let $K$ be the number of subsets $\mathcal{S}$ with at most $k$ elements. Then, $K=\sum_{m=0}^k \binom{d}{m}$. From McDiarmid's inequality, for any $\epsilon' \in (0,1)$ 
\begin{align}\label{eq:chernoff_S} 
\PP\Big\{ \max_{\mathcal{S}: |\mathcal{S}|\leq k} \big|\fbarS-\fS \big|\geq \epsilon' \Big\}\leq 2K \exp\big\{-\frac{n\epsilon'^2}{2}\big\},
\end{align}
where we also used the union bound. As a result, with probability at least $(1-\delta)$, $\max_{\mathcal{S}: |\mathcal{S}|\leq k} \big|\fbarS-\fS \big| \leq \sqrt{\frac{2}{n }\log \frac{2K}{\delta}}$. For $k\leq d/2$, we obtain that 
$$K=\sum_{m=0}^k \binom{d}{m}\leq 1+ k \frac{d^k}{k!}.$$
This implies that the error bound is $O(\sqrt{\frac{1}{n }\log \frac{d^k}{(k-1)!\delta}})$.
Hence, for any $k$-element subset $\mathcal{J}$, with probability at least $(1-\delta)$, we have that
\begin{align}\label{eq:bound on V}
\norm{\PiJ-\Pibar}_2^2\leq O\Big( \frac{2^k}{n}\log \frac{d^k}{(k-1)!\delta}\Big).
\end{align}
%and the proof is complete by taking the square root of both sides.
%\end{proof}






























==> Proofs/proof_lem_mean_est_eff.tex <==
\begin{proof}
Recall that the function $\Pibar$ is defined as $\Pibar(x^d)\deq \sum_{\mathcal{S}: |\mathcal{S}|\leq k} \fbarS \pS(x^d),$ where the Fourier-estimates $ \fbarS$ are defined as $ \fbarS \deq \frac{1}{n}\sum_{i} Y(i) \pS(X(i)).$
From triangle inequality for $\infty$-norm and the definition of $\Piest$ and $\Pibar$ we obtain 
\begin{align}\label{eq:fhatJ fbarJ}
 \norm{\Piest-\Pibar}^2_2 &\leq \sum_{\mathcal{S}: |\mathcal{S}|\leq k} \norm{\festS ~\pestS - \fbarS~ {\psi}_S  }_\infty.
 \end{align} 
 Again by triangle inequality and by adding and subtracting $\fbarS \pestS$, we obtain that 
 \begin{align*}
 \norm{\festS ~\pestS - \fbarS~ {\psi}_S  }_\infty &\leq \norm{\festS ~\pestS - \fbarS ~\pestS  }_\infty +  \norm{\fbarS ~\pestS - \fbarS~ {\psi}_S  }_\infty\\
  &= |\festS-\fbarS|~\norm{\pestS}_\infty + |\fbarS|~ \norm{\pestS - {\psi}_S  }_\infty.
 \end{align*}
 %
 Next, note that from triangle inequality
\begin{align*}
|\festS-\fbarS|\leq \frac{1}{n}\sum_{i}|\pestS(\mathbf{x}(i))-\pS(\mathbf{x}(i))|\leq \norm{\pS-\pestS}_{\infty}.
\end{align*}
Therefore,  
\begin{align}\label{eq:fhatS phihatS}
 \norm{\festS ~\pestS - \fbarS~ {\psi}_S  }_\infty &\leq \big( \norm{\pestS}_\infty + |\fbarS|\big) \norm{\pestS - {\psi}_S  }_\infty.
\end{align}
 We proceed by bounding each term above. 
 As for the first term we have, that $\norm{\pestS}_\infty\leq \norm{\pS}_\infty+\norm{\pestS-\pS}_\infty$. 
% \begin{align*}
%\norm{\pestS}_2^2 = \EE[\pestS(\bfX)^2] = \prod_{j\in \mathcal{S}} \frac{\EE[(X_j-\hat{\mu}_j)^2]}{\hat{\sigma}_j^2} = \prod_{j\in \mathcal{S}}\frac{\sigma_j^2 + (\mu_j - \hat{\mu}_j)^2}{\hat{\sigma}_j^2} = \prod_{j\in \mathcal{S}} \big(b_{\{j\}}^2+d^2_{\{j\}}\big),
% \end{align*}
% where for any subset $\mathcal{A}\subseteq [d]$, define $b_{\mathcal{A}}\deq \prod_{j\in \mathcal{A}}(\frac{\sigma_j}{\hat{\sigma}_j})$  and $d_{\mathcal{A}}\deq \prod_{l\in \mathcal{A}}(\frac{|\mu_l-\hat{\mu}_l|}{\hat{\sigma}_l})$. Let $\epsilon=\frac{2 \epsilon_0}{ \sigma_j^2}$. From the assumptions in the lemma   $b_{\{j\}} \in (1\pm \epsilon)$ and $d_{\{j\}}\in (0, \frac{\epsilon}{\hat{\sigma}_j})$. Therefore, from the inequality $\sigma_j\leq \hat{\sigma}_j (1+\epsilon)$, we get that
% \begin{align*}
%(b_{\{j\}}^2+d_{\{j\}}^2)\leq 1+\epsilon^2+2\epsilon+\frac{\epsilon(1+\epsilon)}{{\sigma}_j}\leq 1+\epsilon',
% \end{align*}
%where $\epsilon' = (3\epsilon+\frac{\epsilon(1+\epsilon)}{{\sigma}_{\min}})$ with  $\sigma_{\min} = \min_j \sigma_j$. Therefore, by taking product of the above terms over $j\in \mathcal{S}$, we get 
% \begin{align*}
%\prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2) \leq (1+ \epsilon')^{|\mathcal{S}|} \leq e^{k\epsilon'},
% \end{align*}
% where the last inequality holds as $|S|\leq k$ and from the fact that $(1+x)\leq e^x$ for all $x\in \RR$. As a result, we get the bound $\norm{\pestS}_2 \leq  e^{\frac{k}{2}\epsilon'}$.
%
 As for the second term, we have 
 \begin{align*}
 \fbarS = \frac{1}{n}\sum_i Y(i) \pS(\bfX(i)) \leq \norm{\pS}_\infty.
 \end{align*}
 Lastly, using the triangle inequality, we obtain from \eqref{eq:fhatS phihatS} that 
\begin{align*}
\norm{\festS ~\pestS - \fbarS~ {\psi}_S  }_\infty &\leq \big(2 \norm{\pS}_\infty + \norm{\pestS-\pS}_\infty  \big) \norm{\pestS - {\psi}_S  }_\infty\\
&\leq \big(2 \norm{\pS}_\infty + \varepsilon \norm{\pS}_\infty  \big) \varepsilon \norm{\ptS  }_\infty\\
&\leq   \varepsilon(2+\varepsilon)\norm{\ptS}^2_\infty\\
&\leq   \varepsilon(2+\varepsilon)c_k. 
\end{align*}
Lastly, from \eqref{eq:fhatJ fbarJ} we get the following bound
\begin{align*}
\norm{\Piest-\Pibar}_\infty&\leq \frac{d^k}{(k-1)!} \varepsilon (2+\varepsilon)c_k.
\end{align*}
With that, the proof is complete. 
\end{proof} 
 
 
 


==> Proofs/proof_lem_mismatch.tex <==
\section{Proof of Lemma \ref{lem:kjunta_nonbinary}}\label{app:proof lem mismatch}
\begin{proof}
Fix a $k$-element subset $\mathcal{J}\subseteq [d]$  and  let $g:\pmm^d\mapsto \pmm$ be a $k$-junta that depends on the coordinates of $\mathcal{J}$. From \eqref{eq:error and inner prod} its generalization loss can be written as  $\PP\big\{Y\neq g(\bfX)\big\}=\frac{1}{2}-\frac{1}{2}\<Y, g\>_D$. Next, consider the collection of all bounded real-valued functions  whose output depends only on the coordinate $\mathcal{J}$. It is not difficult to check that this collection forms a subspace inside the original Hilbert space. Therefore, $g$ belongs to this subspace. Further, as $\PiJ$ minimizes the $\mathcal{L}_2$-distance with $Y$, it is the \textit{projection} of $Y$ onto this space. This implies that inner product $\<Y, g\>_D$ equals to $\<\PiJ, g\>_D$. Hence, the generalization loss of $g$ satisfies the following  
\begin{align*}
\prob{Y\neq g(\bfX)}&=\frac{1}{2}-\frac{1}{2}\<\PiJ, g\>_D \geq \frac{1}{2}-\frac{1}{2}\<|\PiJ|, |g|\>_D\geq \frac{1}{2}-\frac{1}{2}\norm{\PiJ}_{1,D},
\end{align*}
where the last inequality follows as $|g(\bfx)|=1$. Therefore, maximizing over all $k$-element subsets $\mathcal{J}$ gives the bound 
%\begin{align*}
$\Pek \geq \frac{1}{2}-\frac{1}{2}\max_{\mathcal{J}: |\mathcal{J}|= k}\norm{\PiJ}_{1,D}$.
%\end{align*}
Hence, we established a lower-bound on $\Pek$. Next, we show that this bound is achievable.  For that construct a $k$-junta as $g=\sign[\PiJ]$ where $\mathcal{J}$ is a $k$-element subset of $[d]$. Then, from the above argument, the generalization error of such $g$ equals
\begin{align*}
\prob{Y\neq \sign[\PiJ]} &=\frac{1}{2}-\frac{1}{2}\<\PiJ, \sign[\PiJ]\>_D =  \frac{1}{2}-\frac{1}{2}\norm{\PiJ}_{1,D},
\end{align*}
where the last equality follows due to the identity $\<h, \sign[h]\>= \norm{h}_1$ for any function $h$. 
Therefore, optimizing over $\mathcal{J}$ gives 
%\begin{align*}
$\Pek \leq \frac{1}{2}-\frac{1}{2}\max_{\mathcal{J}: |\mathcal{J}|\leq k}\norm{\PiJ}_{1,D}$.
%\end{align*}
As a result,we established an upper-bound that matches with the lower-bound.
\end{proof}

==> Proofs/proof_lem_norm2sign_v1.tex <==
%\section{Proof of Lemma \ref{lem:norm2 sign}}\label{app:proof norm2 sign}

\begin{proof}
From \eqref{eq:error and inner prod} in the main text, the generalization error of $\sign[\hJ]$ can be written as $\frac{1}{2}-\frac{1}{2}\<Y,\sign[\hJ]\>$. Since $\sign[\hJ]$ is a function depending only on the coordinates of $\mathcal{J}$, then in the inner product, we can replace $Y$ with $\PiJ$. We can do that as $\PiJ$ is the projection of $Y$ onto the space of all functions on coordinates $\mathcal{J}$. Hence, we obtain that
\begin{align}\nonumber
\PP\Big\{Y&\neq  \sign[
\hJ(\bfX)]\Big\} = \frac{1}{2}-\frac{1}{2}\<\PiJ,\sign[\hJ]\>\\\label{eq:pe 2 norm stoch}
 &= \frac{1}{4}\big(1-\norm{\PiJ}_2^2+\norm{\PiJ-\sign[\hJ]}_2^2\big).
\end{align}
   The $2$-norm quantity above is upper-bounded as follows
\begin{align*}
 &\norm{\PiJ-\sign[\hJ]}_2^2  \stackrel{(a)}{\leq} \Big(\norm{\PiJ-\hJ}_2+\norm{\hJ-\sign[\hJ]}_2\Big)^2,\\\numberthis \label{eq:mismatch_2norm}
 &\qquad = \Big(\norm{\PiJ-\hJ}^2_2+\norm{\hJ-\sign[\hJ]}^2_2\\
 &\qquad+2\norm{\PiJ-\hJ}_2\norm{\hJ-\sign[\hJ]}_2 \Big),
\end{align*}
where $(a)$  follows from the Minkowski's inequality for $2$-norm.  Note that  $|\hJ-\sign[\hJ]|= |1-|\hJ||.$ Therefore,
\begin{align*}
\norm{\hJ-\sign[\hJ]}^2_2&=\EE\left[(1-|\hJ({X^{\mathcal{J}}})|)^2\right]\\\numberthis\label{eq:fbar-sign}
&= 1+\norm{\hJ}_2^2-2\norm{\hJ}_1.
\end{align*}
From this relation and equations \eqref{eq:pe 2 norm stoch},  \eqref{eq:mismatch_2norm}, we obtain the following upper bound
\begin{align}\nonumber
4\PP\Big\{Y&\neq \sign[
\hJ(\bfX)]\Big\} \leq 2-2\norm{\hJ}_1+ \underbrace{ \norm{\hJ}_2^2- \norm{\PiJ}_2^2}_{\text{(I)}}\\\label{eq:up1}
&~~+\norm{\PiJ-\hJ}^2_2 +2\norm{\PiJ-\hJ}_2\underbrace{\norm{\hJ-\sign[\hJ]}_2}_{\text{(II)}}. 
\end{align}
In what follows, we bound the terms denoted by (I) and (II).\\
\noindent\textbf{Bounding (I):} From the Minkowski's inequality for $2$-norm, we have
\begin{align*}
\norm{\hJ}_2^2 &\leq \Big(\norm{\PiJ}_2+\norm{\hJ-\PiJ}_2  \Big)^2\\
&=\norm{\PiJ}^2_2+\norm{\hJ-\PiJ}^2_2+2\norm{\PiJ}_2 \norm{\hJ-\PiJ}_2\\
&\leq \norm{\PiJ}^2_2+{\norm{\hJ-\PiJ}^2_2+2 \norm{\hJ-\PiJ}_2}
\end{align*}
where the second inequality is due Bessel's inequality implying that $\norm{\PiJ}_2\leq 1$. Hence, the term (I) in \eqref{eq:up1} is upper bounded as
\begin{align}\label{eq:bound on (I)}
\text{(I)}\leq \lambda_1\deq \norm{\hJ-\PiJ}^2_2+2 \norm{\hJ-\PiJ}_2.
\end{align}


\noindent\textbf{Bounding (II):} From \eqref{eq:fbar-sign}, we have
\begin{align*}
&\norm{\hJ-\sign[\hJ]}_2^2 = 1+\norm{\hJ}_2^2-2\norm{\hJ}_1\\
&\stackrel{(a)}{\leq} 1+ 2( \norm{\PiJ}^2_2+ \norm{\PiJ-\hJ}^2_2)-2\norm{\hJ}_1\\
&\stackrel{(b)}{=} 1+ 2( \norm{\PiJ}^2_2+ \norm{\PiJ-\hJ}^2_2)-2\big(\norm{\PiJ}_1+ ( \norm{\hJ}_1-\norm{\PiJ}_1)\big)\\
&= 1+ 2( \norm{\PiJ}^2_2- \norm{\PiJ}_1)+ 2 \norm{\PiJ-\hJ}^2_2-2\big( \norm{\hJ}_1-\norm{\PiJ}_1\big)\\
&\stackrel{(c)}{\leq}  1+ 2 \norm{\PiJ-\hJ}^2_2-2\big( \norm{\hJ}_1-\norm{\PiJ}_1\big)\\\numberthis \label{eq:temp1}
&\stackrel{(d)}{\leq } 1+ 2 \norm{\PiJ-\hJ}^2_2+2\norm{\PiJ-\hJ}_2,
\end{align*}
where $(a)$ follows from the Minkowski's inequality for $2$-norm and the inequality $(x+y)^2\leq 2(x^2+y^2)$. Equality $(b)$ follows by adding and subtracting  $\norm{\PiJ}_1$. Inequality $(c)$ holds as $|\PiJ(x)|\leq 1$ implying that $\norm{\PiJ}^2_2\leq  \norm{\PiJ}_1$. Lastly,  $(d)$ holds because of the following chain of inequalities
\begin{align}\label{eq:normdiff_leq_eps}
\Big|\norm{\PiJ}_1-\norm{\hJ}_1\Big| \leq \norm{\PiJ-\hJ}_1\leq \norm{\PiJ-\hJ}_2,
\end{align}
where the first  is due to the Minkowski's inequality for $1$-norm and 
the second  is due to Holder's. 

Next, we show that the quantity $\big\| \hJ-\sign[h_\mathcal{J}]\big\|_2$ without the square is upper bounded by the same term as in the right-hand side of \eqref{eq:temp1}. That is 
\begin{align}\label{eq:bound on (II)}
\text{(II)} &= \big\| \hJ-\sign[h_\mathcal{J}]\big\|_2\leq \lambda_2\deq 1+ 2 \norm{\PiJ-\hJ}^2_2+2\norm{\PiJ-\hJ}_2.
\end{align}
The argument is as follows: if $\big\| \hJ-\sign[h_\mathcal{J}]\big\|_2$  is 
less than one, then the upper bound holds trivially as $\lambda_2\geq 1$; 
otherwise, this quantity is less than its squared and, hence, the upper-bound holds.  

As a result of the bounds in \eqref{eq:up1}, \eqref{eq:bound on (I)}, and \eqref{eq:bound on (II)} we obtain that 
\begin{align*}
4\PP\Big\{Y &\neq \sign[\hJ(\bfX)]\Big\}  \leq 2-2\norm{\hJ}_1+ \lambda_1+\norm{\PiJ-\hJ}^2_2+  2 \lambda_2 \norm{\PiJ-\hJ}_2\\
&= 2-2\norm{\PiJ}_1+\Big(\norm{\PiJ}_1-\norm{\hJ}_1\Big)  +\lambda_1+\norm{\PiJ-\hJ}^2_2+ 2 \lambda_2 \norm{\PiJ-\hJ}_2\\
&\leq 2-2\norm{\PiJ}_1+\norm{\PiJ-\hJ}_2+ \lambda_1+\norm{\PiJ-\hJ}^2_2+  2 \lambda_2 \norm{\PiJ-\hJ}_2,
\end{align*}
where the last inequality is due to \eqref{eq:normdiff_leq_eps}. Therefore, from the definition of $\lambda_1$ and $\lambda_2$, and the function $U$ in the statement of the lemma, we obtain 
\begin{align*}
4\PP\Big\{Y\neq \sign[
\hJ(\bfX)]\Big\}  \leq 2-2\norm{\PiJ}_1+4U(\norm{\PiJ-\hJ}_2).
\end{align*}
This completes the proof.
\end{proof}


==> Proofs/proof_prop_pstar_Fourier.tex <==
\section{Proof of Proposition \ref{prop:pstar in Fourier}}\label{proof:prop:pstar in Fourier}
Any polynomial $p$ of degree upto $k$ can be written in terms of the monomials $\chi_{\mathcal{S}}$ of degree up to $k$. From the ordering in \eqref{eq:subset_ordering} and the orthogonalization process, these monomials are themselves decompose in terms of the basis $\ptS$ with $|\mathcal{S}|\leq k$. This is done be reversing the recursive equations in the orthogonalization process. Consequently, the polynomial $p$ decomposes as 
\begin{align*}
p\equiv \sum_{\mathcal{S}: |\mathcal{S}|\leq k} p_{\mathcal{S}} \ptS.
\end{align*}
From the Parseval's identity, we have that 
\begin{align*}
\norm{Y-p}_{2,D}^2 &= \sum_{\mathcal{S}} (\alpha_{\mathcal{S}} - p_{\mathcal{S}} )^2\\
&= \sum_{\mathcal{S}: |\mathcal{S}|\leq k} (\alpha_{\mathcal{S}} - p_{\mathcal{S}} )^2 + \sum_{\mathcal{S}: |\mathcal{S}|> k} (\alpha_{\mathcal{S}})^2
\end{align*}
where $\alpha_{\mathcal{S}} = \<Y, \ptS\>_D$ are the Fourier coefficients corresponding to $Y$. The second equality follows since the Fourier expansion of $p$ is zero for $\mathcal{S}$ with $|\mathcal{S}|>k$. As the above equation holds for all $p\in \mathcal{P}_k$, only the first term will be changed. Therefore, the least square error is obtained by setting $p_{\mathcal{S}}=\alpha_{\mathcal{S}}$ for all $\mathcal{S}$ with $|\mathcal{S}| \leq k$. Hence, the optimal polynomial $p^*$ decomposes as 
\begin{align*}
p^*\equiv \sum_{\mathcal{S}: |\mathcal{S}|\leq k} \alpha_{\mathcal{S}} \ptS.
\end{align*}
The proof is complete by noting that $\alpha_{\mathcal{S}} = \<Y, \ptS\>_D$ .

==> Proofs/proof_prop_pstar_in_Fourier.tex <==
\section{Proof of Proposition \ref{prop:pstar in Fourier}}\label{proof:prop:pstar in Fourier}
Any polynomial $p$ of degree upto $k$ can be written in terms of the monomials $\chi_{\mathcal{S}}$ of degree up to $k$. From the ordering in \eqref{eq:subset_ordering} and the orthogonalization process there, these set of monomials can be written in terms of the basis $\ptS$ with $|\mathcal{S}|\leq k$. Consequently, the polynomial $p$ decomposes as 
\begin{align*}
p\equiv \sum_{\mathcal{S}: |\mathcal{S}|\leq k} p_{\mathcal{S}} \ptS.
\end{align*}
From the Parseval's identity, we have that 
\begin{align*}
\norm{Y-p}_{2,D}^2 &= \sum_{\mathcal{S}} (\alpha_{\mathcal{S}} - p_{\mathcal{S}} )^2\\
&= \sum_{\mathcal{S}: |\mathcal{S}|\leq k} (\alpha_{\mathcal{S}} - p_{\mathcal{S}} )^2 + \sum_{\mathcal{S}: |\mathcal{S}|> k} (\alpha_{\mathcal{S}})^2
\end{align*}
where $\alpha_{\mathcal{S}} = \<Y, \ptS\>_D$ are the Fourier coefficients corresponding to $Y$. The second equality follows since the Fourier expansion of $p$ is zero for $\mathcal{S}$ with $|\mathcal{S}|>k$. As the above equation holds for all $p\in \mathcal{P}_k$, only the first term will be changed. Therefore, the least square error is obtained by setting $p_{\mathcal{S}}=\alpha_{\mathcal{S}}$ for all $\mathcal{S}$ with $|\mathcal{S}| \leq k$. 


==> Proofs/proof_thm_low_degree_concentrated.tex <==
%proof of theorem low degree concentrated}
\begin{proof}
We prove the theorem by characterizing the effect of $2$-norm estimation on the error probability. Let
\begin{align*}
{p}^*=\argmin_{p\in \Pk} \norm{Y-p}^2_{2,D}.
\end{align*}
 %that is $$\hat{p}=\argmin_{p:\degree(p)\leq k} \frac{1}{n}\sum_i \big(y_i-p(\bfx_i)\big)^2.$$
%Further, let $${p}^*=\argmin_{p:\degree(p)\leq k} \EE\big[(Y-p(\bfX))^2\big].$$  
 From the second equality in \eqref{eq:error and inner prod}, the generalization error of $\hat{g}$ in Algorithm \ref{alg:fourier} satisfies 
\begin{align}\nonumber
\PP\Big\{Y\neq \hat{g}(\bfX)&\Big\}=\frac{1}{4}\norm{Y-\hat{g}}_{2, D}^2\\\nonumber
&\leq \frac{1}{4}\Big( \norm{Y-p^*}_{2, D}+\norm{p^*-\hat{g}}_{2, D}\Big)^2\\\label{eq:y_neq_ghat_D}
&\leq  \frac{1}{2}\Big(\norm{Y-{p}^*}_{2, D}^2 +\norm{p^*-\hat{g}}_{2, D}^2\Big),
\end{align}
where the  inequality follows from Minkowski's inequality for 2-norm. Observe that \eqref{eq:y_neq_ghat_D} is an upper bound on the generalization error in terms of $2$-norm quantities. Since $p^*$ minimizes the square loss, the first term in \eqref{eq:y_neq_ghat_D} equals
\begin{align*}
\norm{Y-{p}^*}_{2, D}^2 = 1-\norm{{p}^*}_{2}^2.
\end{align*}
We proceed by bounding the second term in \eqref{eq:y_neq_ghat_D}.  From Minkowski's inequality for $2$-norm and by adding and subtracting $\Piest$ as in Algorithm \ref{alg:fourier}, we have that
\begin{align}\nonumber
\norm{p^*-\hat{g}}^2_{2}&\leq \norm{p^*-\Piest}^2_{2}+\norm{\Piest - \hat{g}}^2_2\\\label{eq:pstar-ghat}
&+2\norm{p^*-\Piest}_{2}\norm{\Piest - \hat{g}}_2.
\end{align}
The first term in \eqref{eq:pstar-ghat} is bounded from Lemma \ref{lem:Pi_Y est}. As a result, $\norm{p^*-\Piest}_{2} = \epsilon'_n$, where $$\epsilon'_n = O\Big(\sqrt{\frac{ d^k c_k}{(k-1)!n }\log \frac{4d^k}{(k-1)!\delta}}\Big),$$ with probability at least $(1-\delta)$.  As for the second term in \eqref{eq:pstar-ghat}, we use the identity  $|h-\sign[h]|= |1-|h||$ for any function $h$. Therefore, as $\hat{g}=\sign[\Piest]$, we obtain that
\begin{align}\nonumber
\norm{\Piest - \hat{g}}_2^2&=\EE\left[(1-|\Piest(\bfX)|)^2\right]\\\label{eq:Pihat-ghat}
&= 1+\norm{\Piest}_{2}^2-2\norm{\Piest}_{1}.
\end{align}
Next, we show that the third term in \eqref{eq:pstar-ghat} is less than $4\epsilon'_n$. It suffices to show that $\norm{\Piest - \hat{g}}_2\leq 2$. For that, we use the equality in \eqref{eq:Pihat-ghat}.  By removing the last term in \eqref{eq:Pihat-ghat} and taking the square root we have  
\begin{align*}
\norm{\Piest - \hat{g}}_2 \leq  \sqrt{ 1+\norm{\Piest}_{2}^2}.
\end{align*}
 From the Minkowski's inequality we have that
\begin{align*}
\norm{\Piest}_2&\leq \norm{p^*}_2+\norm{p^*-\Piest}_2\\
& \leq  \norm{p^*}_2+\epsilon_n'\leq 1+\epsilon'_n.
\end{align*}
Hence, we get the desired bound $\norm{\Piest - \hat{g}}_2\leq \sqrt{1+(1+\epsilon'_n)^2}\leq 2$, assuming that $\epsilon'_n\leq 1/3$.
Combining the bounds for each term in \eqref{eq:pstar-ghat}, we get 
\begin{align*}
\norm{p^* - \hat{g}}_2^2&\leq {\epsilon'_n}^2+
1+\norm{\Piest}_{2}^2-2\norm{\Piest}_{1} + 4\epsilon'_n\\
&\leq 1+\norm{\Piest}_{2}^2-2\norm{\Piest}_{1} + 5\epsilon'_n.
\end{align*}
We plug this inequality in \eqref{eq:y_neq_ghat_D}. After rearranging the terms by adding and subtracting $\norm{p^*}_1$,  we obtain the following inequality
\begin{align*}
\PP\Big\{Y\neq \hat{g}&(\bfX)\Big\}\leq \frac{1}{2}\Big(2-2 \norm{p^*}_1+5\epsilon'_n\\
&+2\big(\norm{p^*}_1-\norm{\Piest}_1\big)+ \big(\norm{\Piest}_{2}^2 - \norm{p^*}_{2}^2\big)\Big)\\
&\leq 2\Pek+2\epsilon +5\epsilon'_n,
\end{align*}
where the last inequality follows from Lemma \ref{lem:popt bound norm 1} and the following argument for bounding the last two terms in the first inequality: 

For the $1$-norm difference, the Minkowski's inequality for $1$-norm gives
\begin{align*}
\norm{p^*}_1-\norm{\Piest}_1 \leq \norm{p^*-\Piest}_1 \leq \norm{p^*-\Piest}_2=\epsilon'_n,
\end{align*}
where the last inequality follows from the Jensen's inequality implying that $\norm{\cdot}_1\leq \norm{\cdot}_2$. 

For the difference of square of $2$-norms, we apply the Minkowski's inequality for $2$-norm and obtain
\begin{align*}
\norm{\Piest}_{2}^2 &\leq \norm{p^*}_{2}^2+\norm{p^*-\Piest}_{2}^2+2\norm{p^*}_{2}\norm{p^*-\Piest}_{2}\\
&\leq \norm{p^*}_{2}^2+3 \epsilon'_n.
\end{align*}
where the last inequality holds as $\norm{p^*}_{2}\leq 1$. %The proof is complete by replacing the definition of $\epsilon'_n$.
% and by the inequality $\frac{d^k}{(k-1)!} \leq \sqrt{\frac{k}{2\pi}}(\frac{ed}{k})^k$ which follows from a Stirling type lower bound on $a!$.  
%
\end{proof}

==> proof_lem_popt_norm1.tex <==
\begin{proof}
From \eqref{eq:error and inner prod} the $0-1$ loss of any function $c\in \mathcal{C}$ can be written as $\prob{Y\neq c(\bfX)}=\frac{1}{2}-\frac{1}{2}\<Y,c\>.$   Let $p\in \Pk$ be such that $\norm{c-p}_{2,D}\leq \epsilon$. 
Then, by adding and subtracting $p$, we obtain that
\begin{align}\nonumber
\<Y, c\> &= \<Y, p\> + \<Y, (c-p)\>\\\label{eq:Y,c}
&\leq \<Y, p\> + \norm{Y}_2 \norm{c-p}_2\leq \<Y, p\> + \epsilon,
\end{align}
where the first inequality follows from Cauchy–Schwarz inequality and the second inequality follows because $\norm{Y}_2=1$.  
Note that $\Pk$, the set of all polynomials on $\mathcal{X}$ 
with degree up to $k$, is a (finite-dimensional) subspace inside the Hilbert space $\LD$. Therefore, it has an orthonormal basis denoted by $\{\Psi_1, \Psi_2, ..., \Psi_m\}$, where $m$ is less than $O(d^k)$. 
As a result, the polynomial $p$ can be written as $p\equiv \sum_{j=1}^m \<p,\Psi_j\> \Psi_j$. Hence, 
\begin{align*}
\<Y, p\> = \sum_{j=1}^m \<p,\Psi_j\>~ \<Y,\Psi_j\> = \<\Pi_Y, p\>,
\end{align*}
where $\Pi_Y \equiv \sum_{j=1}^m \<Y,\Psi_j\> \Psi_j$ is the \textit{projection} of $Y$ onto this subspace.  Consequently, from the above equality and \eqref{eq:Y,c}, we obtain that
\begin{align*}
\<Y, c\> &\leq \<\Pi_Y, p\> + \epsilon = \<\Pi_Y, c\> + \<\Pi_Y, (p-c)\>+ \epsilon\\
& \leq \<\Pi_Y, c\> + \norm{\Pi_Y}_2 \norm{p-c}_2+ \epsilon\\
&\leq \norm{\Pi_Y}_1 + \norm{\Pi_Y}_2 \norm{p-c}_2+ \epsilon\\
&\leq \norm{\Pi_Y}_1+2\epsilon,
\end{align*}
where the second inequality follows from Cauchy–Schwarz inequality, the third one holds as $|c(\bfx)|=1$ and the last inequality follows from Bessel's inequality, implying  $\norm{\Piy}_2\leq 1$, and the assumption that $\norm{p-c}_2\leq \epsilon$.
Next, we proceed with the following fact about the projection.
\begin{fact}\label{fact:Pi_Y}
$\Pi_Y$ the projection of $Y$ onto $\Pk$ is the polynomial minimizing $\EE\big[\big(Y-p(\bfX)\big)^2\big]$ over all $p\in \Pk$.
\end{fact}
%\begin{proof}
%Let $\{\Psi_1, \Psi_2, ..., \Psi_m\}$ be an orthonormal basis for $\Pk$. Then, the optimization is equivalent to $\inf_{\mathbf{a} \in \RR^m}L(\mathbf{a})$, where $\mathbf{a}=(a_1, a_2, ..., a_m)$ and 
%\begin{align*}
%L(a_1, a_2, ..., a_m) \deq \EE[(Y-\sum_j a_j \Psi_j)^2 ] .
%\end{align*}
%Taking the derivative of $L$ and equating it to zero gives
%\begin{align*}
%\<Y, \Psi_j\> =  \sum_\ell a_\ell ~\<\Psi_j, \Psi_\ell\> = a_j,
%\end{align*}
%where the last equality follows as $\Psi_j$'s are orthonormal. With this argument the minimizing polynomial is $\sum_j \<Y, \Psi_j\>~\psi_j$ which is $\Pi_Y$.
%\end{proof}
The proof is complete by the following fact implying that $\Pi_Y\equiv p^*$.  
\end{proof}
